Fed-ComBat: A Generalized Federated Framework for Batch Effect Harmonization in Collaborative Studies

The use of multi-centric analyses is crucial for obtaining sufficient sample sizes and representative clinical populations in experimental studies. In this setting, data harmonization techniques are typically employed to address systematic biases and ensure the interoperability of the data. State-of-the-art harmonisation approaches are based on the statistical theory of random effect modeling, allowing to account for either linear of non-linear biases and batch effects. However, optimizing these statistical methods generally requires data centralization at some point during the analysis pipeline, therefore introducing the risk of exposing individual patient information while posing significant data governance issues. To overcome this challenge, in this paper we present Fed-ComBat, a federated framework for batch effect harmonization on decentralized data. Fed-ComBat enables the preservation of nonlinear covariate effects without requiring centralization of data and without prior parametric hypothesis on the variables to account for. We demonstrate the effectiveness of Fed-ComBat against a comprehensive panel of existing approaches based on the state-of-the-art ComBat, along with distributed and nonlinear variants. Our experiments are based on extensive simulated data, and on the analysis of multiple cohorts based on 7 neuroimaging studies comprising healthy controls (CI) and subjects with various disorders such as Parkinson's disease (PD), Alzheimer's disease (AD), and autism spectrum disorder (ASD). Our results show that in a federated settings, Fed-ComBat harmonization exhibits comparable results to centralized methods for both linear and nonlinear cases. On real data, harmonized trajectories of the thickness ofthe right hippocampus across lifespan measured on a set of 7 public studies show comparable results between centralized and federated models and are consistent with the literature when using a nonlinear model. The code is publicly available at: https://gitlab.inria.fr/greguig/fedcombat

==> algorithms/dcombat.tex <==
% \begin{algorithm}
% \caption{Federated Standardization algorithm.}
% \label{alg:federated-standardization}
% \begin{algorithmic}[1]
% \vspace{1.5em}
% \Algphase{Phase 1: Compute federated statistics.}
%     \Procedure{FederatedMean}{$\mathbf{\mathbf{x}_i \in \mathbf{X}}$}
%         \For{each site $i$}
%             \State{$\mathbf{TS}_i \gets \sum_{j=1}^{n_i} \mathbf{x}_{ij}$} \Comment{Compute total sum locally.}
%         \EndFor

%         \State{$\mu \gets \sum_{i}^{S} \frac{1}{n_i}  \mathbf{TS}_i$} \Comment{Compute global mean.}
%         \State \textbf{return} $\mathbf{\mu}$
%     \EndProcedure

%     \Procedure{FederatedStandardDeviation}{$\mathbf{x_i} \in \mathbf{x}_i, \mu$}
%             \For{each site $i$}
%                 \State{$\mathbf{TSS}_i \gets \sum_{j=1}^{n_i} (\mathbf{x}_{ij} - \mu)^2$} \Comment{Compute total sum of squares using federated mean.}
%             \EndFor
%             \State{$\sigma \gets \sqrt{ \sum_{i}^{S} \frac{\mathbf{TSS}_i}{n_i} } $} \Comment{Compute global standard deviation.}
%             \State \textbf{return} $\mathbf{\sigma}$
%     \EndProcedure
% \Algphase{Phase 2: Standardize data at each site.}
%     \Procedure{FederatedStandardization}{$\mathbf{x_i} \in \mathbf{x}_i, \mu, \sigma$}
%         \For{each site $i$}
%             \State{$\mathbf{x}_i \gets \frac{\mathbf{x}_i - \mu}{\sigma} $} \Comment{Standardize using global statistics.}
%         \EndFor
%     \EndProcedure
% \end{algorithmic}
% \end{algorithm}




\begin{algorithm}
\caption{\fedcombat}
\label{alg:distributed-combats}
\begin{algorithmic}[1]
\vspace{1.5em}
\Algphase{Phase 1: Basis decomposition (only for \dcombatgam).}
    \Procedure{BasisDecomposition}{$\mathbf{x}_i \in \mathbf{X}$}
        \State{$\mathbf{x}_i \gets \Call{FederatedStandardization}{\mathbf{x}_i}$}
        \For{each site $i$ and phenotype $g$}
            \State{$x_{ig} \gets \phi_g(x_{ig})$} \Comment{Eqn.~\ref{eq:basis-decomposition}.}
        \EndFor
    \EndProcedure

\Algphase{Phase 2: Parameter estimation using distributed L/S.}
\State{Compute global $\alpha, \hat{\gamma}_{i}$ and $\beta$ from $\big(\sum_{i=1}^S \mathbf{X}_i^{\intercal}\mathbf{X}_i \big)^{-1} \big( \sum_{i=1}^S \mathbf{X}_i^{\intercal} \mathbf{Y}_i \big)$}
\State{Share $\alpha$ and $\beta$ back to centers}

\Algphase{Phase 3: Estimate global variability across phenotypes}
% \State{\textbf{Round 2:} Estimate $\sigma_g \forall_g$}
\For{each site $i$ and phenotype $g$}
    \State{$RSS_{ig} \gets \sum_{j=0}^{n_i} (\yijg - \alpha_g - \xijg\beta_g - \hat{\gamma}_{ig})^{2}$}\Comment{Share RSS.}
\EndFor
\State{$\sigma_g^2 \gets \sqrt{ \sum_i^S \frac{RSS_{ig}}{n_i} } $}\Comment{Compute global phenotype variability.}

\Algphase{Phase 4: \combat random effects estimation using EB.}
% \State{\textbf{Round 3:} Compute random effects with EB}
\For{each site $i$ and phenotype $g$}
    \State{$\gammaig^* \sim \mathcal{N}(Y_i, \tau_i^2)$ and $ \deltaig^* \sim \textrm{InverseGamma}(\lambda_i, \vartheta_i)$}
    \While{Convergence}
    \State{$\gammaig^{*} = \frac{n_i \Bar{\tau}_i^2\hat{\gamma}_{ig} + \deltaig^{2*} \Bar{\gamma}_{ig}}{n_i \Bar{\tau}_i^2 + \deltaig^{2*}},  \, \deltaig^{*} = \frac{\Bar{\theta}_i + \frac{1}{2} \sum_{j=1}^{n_i} (z_{ijg} - \gammaig^*)^2}{\frac{n_i}{2} \Bar{\lambda}_i - 1}$}\Comment{Empirical Bayes.}
    % \State{}
    \EndWhile
% \State{Estimate $\gammaig^*, \deltaig^*$and harmonize using eqn~\ref{eqn:harmonize}}
\EndFor


\end{algorithmic}
\end{algorithm}

==> algorithms/fedcombat.tex <==
\todo[inline]{\fedcombat algorithm.}

==> sections/related-works.tex <==
\subsubsection{\dcombat}
\label{sec:dcombat}
\cite{dcombat} proposed a distributed version of \combat that allows correction for batch effects in a distributed manner. This is achieved by taking advantage of the multivariate linear regression problem solved in \combat, requiring to compute the product between the inverse of a covariance matrix and the data-targets cross-covariance. Both can be computed by aggregating the individual matrices provided by each site. This allows us to reformulate \cref{eq:general-combat} as done by \citep{dcombat}:

\begin{align}
\underbrace{\begin{bmatrix}
y_{11g} \\
\vdots \\
y_{ijg} \\
\vdots \\
y_{Sn_sg}
\end{bmatrix}}_{\mathbf{y}_g} = \underbrace{\left[\begin{array}{ccc|ccc|c}
x_{111} & \dots & x_{11C} & 1 & \cdots & 0 & 1 \\
\vdots & x_{ijc} & \vdots & \vdots & \ddots & \vdots & \vdots \\
x_{Sn_S1} & \dots & x_{Sn_sC} & 0 & \dots & 1 & 1
\end{array}\right]}_{\mathbf{X}} \underbrace{\left[\begin{array}{c}
\hat{\theta}_{g1} \\
\vdots \\
\hat{\theta}_{gc} \\ \hline
\hat{\gamma}_{1g} \\
\vdots \\ \hline
\hat{\alpha}_g
\end{array} \right]^{\intercal}}_{\hat{\boldsymbol{\Theta}}_g}+ \boldsymbol{\delta}_g\boldsymbol{\varepsilon}_g
\label{eq:dcombat-formulation}
\end{align}

Starting from the panel formulation where $\mathbf{y_g}$ is the stacked vector of all subjects across all sites $i$, and $\mathbf{X}$ is a design matrix containing the covariate effects to be preserved indexed by $c$ in subject $j$ from site $i$ ($x_{ijc}$), an indicator matrix encoding the site, and a column of ones to capture $\alpha_g$, we can estimate the augmented parameter matrix $\hat{\mathbf{\Theta}}_g$ using maximum likelihood. The estimator can be decomposed as a sum of the covariance and the cross-covariance matrices at each site, as shown in Equation \ref{eqn:matrix-sum-dec}. This formulation has also been used to distribute latent variable models, such as PCA and PLS, among multiple sites \citep{silva2019federated, lorenzi2018susceptibility}. The authors have also suggested sharing a partial-eigen decomposition to mitigate the risk of data leakage, as shown in Equation \ref{eqn:fed-svd} where the least squares problem is decomposed by $\mathbf{X}^{\intercal} \mathbf{X}$ which denotes the covariance matrix, $\mathbf{X}^{\intercal} \mathbf{y}_g$ the cross-covariance matrix for phenotype $g$, $\mathbf{Q}_i, \mathbf{\Lambda}_i$ the eigen decomposition for the covariance matrix in site $i$ and, $\mathbf{U}_i\mathbf{\Sigma}_i\mathbf{V}_i$ the SVD decomposition for the cross-covariance matrix in site $i$.
\begin{eqnarray}
    \hat{\mathbf{\Theta}}_g &=& \big( \mathbf{X}^{\intercal} \mathbf{X} \big)^{-1} \mathbf{X}^{\intercal} \mathbf{y}_g = \Bigg( \sum_{i=1}^{S} \mathbf{X}_i^{\intercal}  \mathbf{X}_i \Bigg)^{-1}  \Bigg( \sum_{i=1}^{S} \mathbf{X}_i^{\intercal} \mathbf{y}_{ig} \Bigg) \label{eqn:matrix-sum-dec}\\
    &=& \Bigg( \sum_{i=1}^{S} \mathbf{Q}_i\mathbf{\Lambda}_i\mathbf{Q}_i^{-1} \Bigg)\Bigg( \sum_{i=1}^{S} \mathbf{U}_i\mathbf{\Sigma}_i\mathbf{V}_i^{\intercal} \Bigg) \label{eqn:fed-svd}
\label{eq:dcombat-analytical}
\end{eqnarray}

